EvoCodeBench: An Evolving Code Generation Benchmark with Domain-Specific Evaluations

How to evaluate Large Language Models (LLMs) in code generation remains an open question. Existing benchmarks have two limitations - data leakage and lack of domain-specific evaluation. The former hurts the fairness of benchmarks, and the latter hinders practitioners from selecting superior LLMs for specific programming domains. To address these two limitations, we propose a new benchmark - EvoCodeBench, which has the following advances: (1) Evolving data. EvoCodeBench will be dynamically updated every period (e.g., 6 months) to avoid data leakage. This paper releases the first version - EvoCodeBench-2403, containing 275 samples from 25 repositories. (2) A domain taxonomy and domain labels. Based on the statistics of open-source communities, we design a programming domain taxonomy consisting of 10 popular domains. Based on the taxonomy, we annotate each sample in EvoCodeBench with a domain label. (3) Domain-specific evaluations. Besides the Pass@k, we compute the Domain-Specific Improvement (DSI) and define LLMs' comfort and strange domains. These evaluations help practitioners select superior LLMs in specific domains and discover the shortcomings of existing LLMs. We evaluate 8 popular LLMs (e.g., gpt-4, DeepSeek Coder) on EvoCodeBench and summarize some insights. EvoCodeBench reveals the actual abilities of these LLMs in real-world repositories. For example, the highest Pass@1 of gpt-4 on EvoCodeBench-2403 is only 20.74%. Besides, we evaluate LLMs in different domains and discover their comfort and strange domains. For example, gpt-4 performs best in most domains but falls behind others in the Internet domain. StarCoder 2-15B unexpectedly performs well in the Database domain and even outperforms 33B LLMs. EvoCodeBench has been released.

==> chapter/Benchmark_Collection.tex <==
\section{Benchmark Collection Pipeline}
\label{sec:benchmark_collection}

We build an automatic pipeline for collecting \bench from the latest repositories. The pipeline consists of four stages as follows.

\textbf{\ding{182} Repository Selection.} We crawl high-quality repositories from GitHub satisfying the following criteria: open-source Python projects; created in recent months; non-fork and non-malicious projects; more than 50 stars; and having explicit unit tests. 

\textbf{\ding{183} Function Parse.} We extract functions from repositories and exclude trivial functions (\eg empty or initialization functions). We extract each function’s signature and function body (\ie reference code). We developed a static analysis-based parser to extract reference dependencies with the reference code.

\textbf{\ding{184} Tests Construction.} For each function, we extract test cases invoking it from current repositories. We use \texttt{pip}\footnote{\url{https://pypi.org/project/pip/}} to automatically install required packages for each repository and leverage \texttt{Pytest}\footnote{\url{https://docs.pytest.org/en/8.0.x/}} to run test cases. Functions without executable test cases are excluded. 

\textbf{\ding{185} Deduplication.} To improve the diversity of \bench, we perform repository-level deduplication based on the Jaccard similarities in code files and imports. The former removes duplicate repositories in text surfaces, and the latter removes repositories in domains that are too similar.

\textbf{\ding{186} Requirement Annotation.} Manually writing requirements is time-consuming and laborious. Inspired by the powerful abilities of LLMs in code comment generation \cite{LLM4CS}, we leverage LLMs to generate natural language requirements. Specifically, we manually craft a few-shot prompt, which teaches LLMs to write requirements in a specific format (\ie functional descriptions and input-output parameters). Appendix \ref{sec:appendix:collection:gen_requirement} the details of prompts.

\textbf{\ding{187} Benchmark Construction.} Finally, we select samples from the outputs of step \ding{186} to construct \bench. We strive to make \bench satisfy the following goals: consistent with the code distribution observed in 500 real-world repositories; close to the average number of dependencies in 500 real-world repositories; including as many samples as possible. 

==> table/Base_LLMs.tex <==
\begin{table}[t]
\caption{Studied LLMs in this paper. Context L.: Context Window.}
\label{tab:Base_LLMs}
\resizebox{\linewidth}{!}{
\begin{tabular}{llcc}
\toprule
Type & Name & Version & Context W. \\ \midrule
\multirow{2}{*}{Closed-source} 
 & gpt-4 & gpt-4-turbo-1106 & 128,000 \\ 
 & gpt-3.5 & gpt-3.5-turbo-1106 & 16,385 \\ \midrule
\multirow{8}{*}{Open-source} 
 & StarCoder 2 & 15B & 16,384 \\
 & StarCoder 2 & 7B & 16,384 \\
 & DeepSeek Coder & 33B & 16,384 \\
 & DeepSeek Coder & 6.7B & 16,384 \\
 & CodeLLaMa & 13B & 16,384 \\
 & CodeLLaMa & 7B & 16,384 \\
 & Gemma & 7B & 8,192 \\
 & Qwen 1.5 & 7B & 32,768 \\
 \bottomrule
\end{tabular}}
\end{table}

==> table/feature_comparison.tex <==
\begin{table}[t]
\caption{The comparison between existing benchmarks and \bench.}
\label{tab:feature_comparison}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccc}
\toprule
Benchmark & Real Repo. & Real Code Distribution & Comprehensive Annota. & Robust Metric & Avoiding Data Leak. \\ \midrule
CoNaLA \cite{CoNaLA} & \faTimes & \faTimes & \faTimes & \faTimes & \faTimes \\
Concode \cite{Concode} & \faCheck & \faTimes & \faTimes & \faTimes & \faTimes \\ 
HumanEval \cite{Codex} & \faTimes & \faTimes & \faTimes & \faTimes & \faTimes \\ 
MBPP \cite{MBPP} & \faTimes & \faTimes & \faTimes & \faTimes & \faTimes \\ 
APPS \cite{APPS} & \faTimes & \faTimes & \faTimes & \faTimes & \faTimes \\
PandasEval \cite{CERT} & \faTimes & \faTimes & \faTimes & \faTimes & \faTimes \\
NumpyEval \cite{CERT} & \faTimes & \faTimes & \faTimes & \faTimes & \faTimes \\
AixBench \cite{SkCoder} & \faCheck & \faTimes & \faTimes & \faTimes & \faTimes \\
ClassEval \cite{ClassEval} & \faTimes & \faTimes & \faTimes & \faTimes & \faTimes \\
LiveCodeBench \cite{LiveCodeBench} & \faTimes & \faTimes & \faTimes & \faTimes & \faCheck \\ 
CoderEval \cite{CoderEval} & \faCheck & \faTimes & \faTimes & \faCheck & \faTimes \\ 
DevEval  & \faCheck & \faCheck & \faCheck & \faCheck & \faTimes \\ 
\midrule
\bench (Ours) & \faCheck & \faCheck & \faCheck & \faCheck & \faCheck \\
\bottomrule
\end{tabular}}
\end{table}
